Utilizing Excess Resources in Training Neural Networks

In this work, we suggest Kernel Filtering Linear Overparameterization (KFLO), where a linear cascade of filtering layers is used during training to improve network performance in test time. We implement this cascade in a kernel filtering fashion, which prevents the trained architecture from becoming unnecessarily deeper. This also allows using our approach with almost any network architecture and let combining the filtering layers into a single layer in test time. Thus, our approach does not add computational complexity during inference. We demonstrate the advantage of KFLO on various network models and datasets in supervised learning.

==> tables/results_TL40_cifar100_from_cifar10.tex <==
\begin{table}
\begin{adjustbox}{width=1.\linewidth}
\begin{tabular}{|l|l|l|l|l|}
\hline
Method                     & {\small wResnet-16-8}         & {\small wResnet-28-2}         & {\small wResnet-28-5}         &  {\small wResnet-28-10}        \\ \hline
vanilla                    & 69.81 ±0.19          & 66.69 ±0.24          & 69.56 ±0.19          & 70.79 ±0.41          \\
vanilla TL  & 71.20 ±0.41          & 67.12 ±0.25          & 71.43 ±0.42          & 73.15 ±0.33          \\
KFLO 2x1                   & 71.50 ±0.23          & 67.06 ±0.53          & 71.04 ±0.27          & 73.11 ±0.26          \\
KFLO 2x1 TL & 71.62 ±0.37          & 67.26 ±0.41          & 71.33 ±0.34          & 72.19 ±0.35          \\
KFLO 2x4                   & 71.86 ±0.14          & 67.66 ±0.34          & \textbf{71.63 ±0.27} & \textbf{73.36 ±0.29} \\
KFLO 2x4 TL & \textbf{71.97 ±0.32} & \textbf{67.85 ±0.32} & 71.60 ±0.22          & 72.55 ±0.26          \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Transfer Learning accuracy results. Only 40\% of the CIFAR-100 training set available. The TL suffix denotes using networks pre-trained on the full CIFAR-10 training set.}
% \caption{Transfer Learning accuracy results. Here training was done using 40\% of the CIFAR-100 training set. The TL suffix denotes experiments where networks pre-trained on the full CIFAR-10 training set are available.}
\label{table:resultsTransferLearning}
\end{table}

==> tables/results_cifar100_abStudy.tex <==
% \begin{table}
% \begin{adjustbox}{width=1.\linewidth}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Method   & {\small wResnet-16-8}         & {\small wResnet-28-2}         &  {\small wResnet-28-5}         & {\small wResnet-28-10}        \\ \hline
% KFLO 2x1 & 79.47 ±0.21          & 75.69 ±0.39          & 79.60 ±0.24          & 81.35 ±0.23          \\
% KFLO 2x2 & 79.68 ±0.31          & 75.91 ±0.31          & 79.76 ±0.22          & 81.36 ±0.15          \\
% KFLO 2x3 & 79.59 ±0.16          & 76.00 ±0.29          & \textbf{79.96 ±0.18} & \textbf{81.46 ±0.15} \\
% KFLO 2x4 & \textbf{79.74 ±0.24} & \textbf{76.07 ±0.29} & \textbf{79.96 ±0.27} & 81.33 ±0.20          \\
% KFLO 3x2 & 76.51 ±0.26          & 68.21 ±0.39          & 75.69 ±0.22          & 78.93 ±0.12          \\ \hline
% \end{tabular}
% \end{adjustbox}
% \caption{CIFAR-100 accuracy results, \OurMethod{} ablation study.}
% % \caption{CIFAR-100 accuracy results for different \OurMethod{} configurations.}
% \label{table:resultsCifar100AbStudy}
% \end{table}
